Synthetic ECG Generation for Data Augmentation and Transfer Learning in Arrhythmia Classification

Deep learning models need a sufficient amount of data in order to be able to find the hidden patterns in it. It is the purpose of generative modeling to learn the data distribution, thus allowing us to sample more data and augment the original dataset. In the context of physiological data, and more specifically electrocardiogram (ECG) data, given its sensitive nature and expensive data collection, we can exploit the benefits of generative models in order to enlarge existing datasets and improve downstream tasks, in our case, classification of heart rhythm. In this work, we explore the usefulness of synthetic data generated with different generative models from Deep Learning namely Diffweave, Time-Diffusion and Time-VQVAE in order to obtain better classification results for two open source multivariate ECG datasets. Moreover, we also investigate the effects of transfer learning, by fine-tuning a synthetically pre-trained model and then progressively adding increasing proportions of real data. We conclude that although the synthetic samples resemble the real ones, the classification improvement when simply augmenting the real dataset is barely noticeable on individual datasets, but when both datasets are merged the results show an increase across all metrics for the classifiers when using synthetic samples as augmented data. From the fine-tuning results the Time-VQVAE generative model has shown to be superior to the others but not powerful enough to achieve results close to a classifier trained with real data only. In addition, methods and metrics for measuring closeness between synthetic data and the real one have been explored as a side effect of the main research questions of this study.

==> leftovers.tex <==

\subsection{TimeGAN}
TimeGAN consists of four network components: an embedding function, recovery function, sequence generator, and sequence discriminator. The key insight is that the autoencoding components (first two) are trained jointly with the adversarial components (latter two). The embedding network provides the latent space, the adversarial network operates wihtin this space, and the latent dynamics of both real and synthetic data are synchronized through a supervised loss. The authors frame the data generation process as follows:
\begin{quote}
Consider the general data setting where each instance consists of two elements: static features (that do not change over time), and temporal features (that occur over time). Let $\mathcal{S}$ be a vector space of static features, $\mathcal{X}$ of temporal features, and let $\textbf{S} \in \mathcal{S}$, $\textbf{X} \in \mathcal{X}$ be random vectors that can be instantiated with specific values denoted $\textbf{s}$ and $\textbf{x}$. We consider tuples of the form $(\textbf{S}, \textbf{X}_{1:T})$ with some joint distribution $p$. The training dataset is thus $ \mathcal{D} = {(\textbf{s}_{n}, \textbf{x}_{n,1:T_{n}})}_{n=1}^{N}$, where individual samples are indexed by $n \in \{1,\text{...}, N\}$.

Our goal is to use the training data $\mathcal{D}$ to learn a density $\hat{p}(\textbf{S}, \textbf{X}_{1:T})$ that best approximates $p(\textbf{S}, \textbf{X}_{1:T})$. This high-level objective is difficult to optimize in the standard GAN framework. Therefore we additionally make use of the autoregressvie decomposition of the joint $p(\textbf{S}, \textbf{X}_{1:T}) = p(\textbf{S} \prod_{t} p(\textbf{X}_{t} | S, \textbf{X}_{1:t-1})$ to focus specially on the conditionals, yielding the complementary objective of learning a density $\hat{p}(\textbf{X}_{t} | \textbf{S}, \textbf{X}_{1:T})$ that best approximates $p(\textbf{X}_{t} | \textbf{S}, \textbf{X}_{1:T})$ at any time $t$ \cite{yoon_2019}.
\end{quote}
Thus, in their framework we are left with two objectives on the sequence-level (matching the joint distribution) which can be broken down into a series of stepwise objectives (matching the conditionals). the first is global,
\begin{equation}
    \min_{\hat{p}} D \Big( p(\textbf{S}, \textbf{X}_{1:T}) || \hat{p}(\textbf{S}, \textbf{X}_{1:T}) \Big)
\end{equation}
where $D$ is some appropriate measure of distance between distributions. The second is local,
\begin{equation}
    \min_{\hat{p}} D \Big( p(\textbf{X}_{t} | \textbf{S}, \textbf{X}_{1:t-1}) || \hat{p}(\textbf{X}_{t}|\textbf{S}, \textbf{X}_{q:t-1}) \Big)
\end{equation}
for any $t$. Under an ideal discriminator in the GAN framework, the former takes the form of the Jensen-Shannon divergence. Using the original data for supervision via maximum-likelihood (ML) training, the latter takes the form of the Kullback-Leibler divergence \cite{yoon_2019}.
% Finish

\subsection{Fourier Flows}
Normalizing flows (NF) are attractive because of their capacity to access explicit likelihoods, which is crucial for applications when uncertainty quantification or anomaly detection is required. It is based on the following change-of-variables formula: 

Let $\textbf{z} \in \mathbb{R}^{D}$ be a random variable with a known tractable probability density function $p(\textbf{z})$, and let $g: \mathbb{R}^{D} \rightarrow \mathbb{R}^{D}$ be an invertible and differentiable mapping with an inverse mapping $ f = g^{-1}$. Let $x = g(\textbf{z})$ be a transformed random variable--the probability density function $p(\textbf{x})$ can be obtained using the change of variable rule as follows, for $\textbf{J}[f]$ and $\textbf{J}[g]$ Jacobian matrices of  functions $f$ and $g$, respectively \cite{alaa2020generative}.

\begin{equation}
    p(\textbf{x}) = p(\textbf{z}) \cdot | \text{det} \ \textbf{J}[g] |^{-1} = p(f(\textbf{x})) \cdot | \text{det} \ \textbf{J} [f] |
\end{equation}

NFs provide an expression for the probability density function of diffeomorphic transformations of a random variable. With carefully chosen transformations, if the initial density is tractable (e.g. Gaussian), the transformed density can be easily manipulated and sampled as well, provided that the Jacobian of the transformation can be computed efficiently \cite{bekri2024timechanged}. More formally, NFs are compositions of $M$ mappings that transform random draws from a predefined distribution $ \textbf{z} \sim p(\textbf{z})$ to a desired distribution $p(\textbf{x})$. A flow comprises a chain of bijective maps $g = g^{(1)} \circ g^{(2)} \circ \cdot \cdot \cdot \circ g^{(M)}$ with an inverse mapping $f = f^{(1)} \circ f^{(2)} \circ \cdot \cdot \cdot \circ f^{(M)}.$ Using the change of variables forumla above and applying the chain rule to the Jacobian of the composition, the log-likelihood of $\textbf{x}$ can be written as \cite{rezende2016variational}:
\begin{equation}
    \text{log} \ p(\textbf{x}) = \text{log} \ p(\textbf{z}) + \sum_{m=1}^{M} \text{log} \ | \text{det} \ \textbf{J} [f_{\textbf{m}}] |.
\end{equation}
Fourier Flows \cite{alaa2020generative} operate on time-series data in the frequency-domain rather than the time-domain. They convert variable-length time series with varying sampling rates across different features to a fixed-size spectral representation using the discrete Fourier transform (DFT), and then learn the distribution of the data in the frequency domain by applying a chain of data-dependent spectral filters to frequency-transformed time series. They are comprised of two steps: a \textbf{frequency transform} layer followed by a data-dependent \textbf{spectral filtering} layer.

In the first step, the time series $\textbf{x} = [\textbf{x}_{0}, \cdot \cdot \cdot, \textbf{x}_{T-1}]$ is transformed into its spectral representation via the DFT operation to each dimension $d$ independently. The data undergoes the following steps during this step: \textit{temporal zero padding}, \textit{Fourier transform}, and \textit{spectral cropping}. The temporal zero-padding step ensures that the time series $\bar{\textbf{x}}^{d}$ and their frequency spectrum $\bar{\textbf{X}}^{d}$ have a fixed length of $N$. 
Since the DFT coefficients are complex-valued, $\bar{\textbf{X}}^{d}$ is a tensor with dimensions $2 \times D \times N$, assuring that $N \geq T$ to guarantee a lossless recovery of $\textbf{x}$ via inverse DFT. 
The spectral cropping discards the $N/2+1^{th}$ to $N^{th}$ frequency components in both $\text{Re}(\bar{\textbf{X}})$ and $\text{Im}(\bar{\textbf{X}})$, since $\textbf{x}$ is real-valued.

In the second step is an \textit{affine coupling layer}, which can be though of as a spectral filtering operation where the frequency tranform of the \textit{even} part of the time series, $\text{Re}(\hat{X})$, is applied to a fiter with a transfer function $\textbf{H}$, which depends on the \textit{odd} part of $\textbf{x}$. This transfer function is implemented through a bi-directional RNN with shared parameters across all different frequency components.
